DIST: Rendering Deep Implicit Signed Distance Function with Differentiable Sphere Tracing

We propose a differentiable sphere tracing algorithm to bridge the gap between inverse graphics methods and the recently proposed deep learning based implicit signed distance function. Due to the nature of the implicit function, the rendering process requires tremendous function queries, which is particularly problematic when the function is represented as a neural network. We optimize both the forward and backward passes of our rendering layer to make it run efficiently with affordable memory consumption on a commodity graphics card. Our rendering method is fully differentiable such that losses can be directly computed on the rendered 2D observations, and the gradients can be propagated backwards to optimize the 3D geometry. We show that our rendering method can effectively reconstruct accurate 3D shapes from various inputs, such as sparse depth and multi-view images, through inverse optimization. With the geometry based reasoning, our 3D shape prediction methods show excellent generalization capability and robustness against various noises.

==> figures/figure_camera_demo.tex <==
\begin{figure}[tb]
\centering
\scriptsize
\setlength\tabcolsep{2.3pt} % default value: 6pt
\begin{tabular}{cccccc}
pred. depth & depth grad. & pred. normal & normal grad. & pred. mask & mask grad.
\\
{\includegraphics[width=0.14\linewidth]{img_src/demo_camera/vis_0_depth_output.png}} &
{\includegraphics[width=0.14\linewidth]{img_src/demo_camera/vis_0_depth_loss.png}} &
{\includegraphics[width=0.14\linewidth]{img_src/demo_camera/vis_0_normal_output.png}} &
{\includegraphics[width=0.14\linewidth]{img_src/demo_camera/vis_0_normal_loss.png}} & 
{\includegraphics[width=0.14\linewidth]{img_src/demo_camera/vis_0_mask_output.png}} &
{\includegraphics[width=0.14\linewidth]{img_src/demo_camera/vis_0_mask_loss.png}}
\\
{\includegraphics[width=0.14\linewidth]{img_src/demo_camera/vis_12_depth_output.png}} &
{\includegraphics[width=0.14\linewidth]{img_src/demo_camera/vis_12_depth_loss.png}} &
{\includegraphics[width=0.14\linewidth]{img_src/demo_camera/vis_12_normal_output.png}} &
{\includegraphics[width=0.14\linewidth]{img_src/demo_camera/vis_12_normal_loss.png}} &
{\includegraphics[width=0.14\linewidth]{img_src/demo_camera/vis_12_mask_output.png}} &
{\includegraphics[width=0.14\linewidth]{img_src/demo_camera/vis_12_mask_loss.png}}
% \\
% {\includegraphics[width=0.14\linewidth]{img_src/demo_camera/vis_35_depth_output.png}} &
% {\includegraphics[width=0.14\linewidth]{img_src/demo_camera/vis_35_depth_loss.png}} &
% {\includegraphics[width=0.14\linewidth]{img_src/demo_camera/vis_35_normal_output.png}} &
% {\includegraphics[width=0.14\linewidth]{img_src/demo_camera/vis_35_normal_loss.png}} &
% {\includegraphics[width=0.14\linewidth]{img_src/demo_camera/vis_35_mask_output.png}} &
% {\includegraphics[width=0.14\linewidth]{img_src/demo_camera/vis_35_mask_loss.png}}
\\
{\includegraphics[width=0.14\linewidth]{img_src/demo_camera/vis_84_depth_output.png}} &
{\includegraphics[width=0.14\linewidth]{img_src/demo_camera/vis_84_depth_loss.png}} &
{\includegraphics[width=0.14\linewidth]{img_src/demo_camera/vis_84_normal_output.png}} &
{\includegraphics[width=0.14\linewidth]{img_src/demo_camera/vis_84_normal_loss.png}} & 
{\includegraphics[width=0.14\linewidth]{img_src/demo_camera/vis_84_mask_output.png}} &
{\includegraphics[width=0.14\linewidth]{img_src/demo_camera/vis_84_mask_loss.png}}
\\
{\includegraphics[width=0.14\linewidth]{img_src/demo_camera/vis_199_depth_output.png}} &
{\includegraphics[width=0.14\linewidth]{img_src/demo_camera/vis_199_depth_loss.png}} &
{\includegraphics[width=0.14\linewidth]{img_src/demo_camera/vis_199_normal_output.png}} &
{\includegraphics[width=0.14\linewidth]{img_src/demo_camera/vis_199_normal_loss.png}} &
{\includegraphics[width=0.14\linewidth]{img_src/demo_camera/vis_199_mask_output.png}} &
{\includegraphics[width=0.14\linewidth]{img_src/demo_camera/vis_199_mask_loss.png}}
\\
\end{tabular}
\vspace{5pt}
\centering
\caption{Illustration of the optimization process over the camera extrinsic parameters. Our differentiable renderer is able to successfully propagate the error from the image plane to the camera.}
\label{fig::demo_camera}
\end{figure}


==> figures/figure_pix3d.tex <==
\begin{figure}[tb]
\centering
\scriptsize
\setlength\tabcolsep{1.5pt} % default value: 6pt
\begin{tabular}{c|c|c|c|c|c}
\hline
Img & ShapeHD \cite{wu2018learning} & Ours & Img & ShapeHD \cite{wu2018learning} & Ours \\
\hline
{\includegraphics[width=35pt, height=35pt]{img_src/demo_pix3d/2300_img.png}} &
{\includegraphics[width=35pt, height=35pt]{img_src/demo_pix3d/shapehd_2300.png}} &
{\includegraphics[width=35pt, height=35pt]{img_src/demo_pix3d/2300.png}} &
{\includegraphics[width=35pt, height=35pt]{img_src/demo_pix3d/25_img.png}} &
{\includegraphics[width=35pt, height=35pt]{img_src/demo_pix3d/shapehd_0025.png}} &
{\includegraphics[width=35pt, height=35pt]{img_src/demo_pix3d/25.png}}
\\
{\includegraphics[width=35pt, height=35pt]{img_src/demo_pix3d/1119_img.png}} &
{\includegraphics[width=35pt, height=35pt]{img_src/demo_pix3d/shapehd_1119.png}} &
{\includegraphics[width=35pt, height=35pt]{img_src/demo_pix3d/1119.png}} &
{\includegraphics[width=35pt, height=35pt]{img_src/demo_pix3d/958_img.png}} &
{\includegraphics[width=35pt, height=35pt]{img_src/demo_pix3d/shapehd_0958.png}} &
{\includegraphics[width=35pt, height=35pt]{img_src/demo_pix3d/958.png}}
\\
{\includegraphics[width=35pt, height=35pt]{img_src/demo_pix3d/2709_img.png}} &
{\includegraphics[width=35pt, height=35pt]{img_src/demo_pix3d/shapehd_2709.png}} &
{\includegraphics[width=35pt, height=35pt]{img_src/demo_pix3d/2709.png}} &
{\includegraphics[width=35pt, height=35pt]{img_src/demo_pix3d/1011_img.png}} &
{\includegraphics[width=35pt, height=35pt]{img_src/demo_pix3d/shapehd_1011.png}} &
{\includegraphics[width=35pt, height=35pt]{img_src/demo_pix3d/1011.png}}
\\
\hline
\end{tabular}
\vspace{5pt}
\centering
\caption{Qualitative results on Pix3D \cite{sun2018pix3d} dataset. Our method can predict high-quality image-aligned shapes on real-world data.}
\label{fig::pix3d}
\end{figure}


==> figures/figure_render_pipeline.tex <==
\begin{figure*}[tb]
\centering
\scriptsize
\setlength\tabcolsep{2.3pt} % default value: 6pt
\includegraphics[\linewidth]{img_src/render_pipeline.jpg}
\centering
\caption{The rendering pipeline.}
\label{fig::render_pipeline}
\end{figure*}


==> figures/mv_comp_pmo.tex <==

\begin{figure}[!htb]
\centering
\scriptsize
\setlength\tabcolsep{2.3pt} % default value: 6pt
\begin{tabular}{cccc}
Video sequence & PMO (rand init)& PMO & \textbf{Ours}
\\
{\includegraphics[width=0.25\linewidth]{img_src/mv_comp_pmo/plane_14_rgb.png}} &
{\includegraphics[width=0.22\linewidth]{img_src/mv_comp_pmo/plane_14_pmo_noise.png}} &
{\includegraphics[width=0.22\linewidth]{img_src/mv_comp_pmo/plane_14_pmo.png}} &
{\includegraphics[width=0.22\linewidth]{img_src/mv_comp_pmo/plane_14_ours.png}}
\\
% {}&{35.744 / 12.213}&{6.656 / 0.505}&{1.425 / 0.397}\\
{\includegraphics[width=0.25\linewidth]{img_src/mv_comp_pmo/plane_9_rgb.png}} &
{\includegraphics[width=0.22\linewidth]{img_src/mv_comp_pmo/plane_9_pmo_noise.png}} &
{\includegraphics[width=0.22\linewidth]{img_src/mv_comp_pmo/plane_9_pmo.png}} &
{\includegraphics[width=0.2\linewidth]{img_src/mv_comp_pmo/plane_9_ours.png}}
\\
% {}&{20.754 / 5.411}&{0.486 / 0.164}&{1.186 / 0.534}\\
{\includegraphics[width=0.25\linewidth]{img_src/mv_comp_pmo/car_19_rgb.png}} &
{\includegraphics[width=0.22\linewidth]{img_src/mv_comp_pmo/car_19_pmo_noise.png}} &
{\includegraphics[width=0.22\linewidth]{img_src/mv_comp_pmo/car_19_pmo.png}} &
{\includegraphics[width=0.22\linewidth]{img_src/mv_comp_pmo/car_19_ours.png}}
\\
% {}&{2.186 / 0.943}&{1.070 / 0.635}&{1.143 / 0.426}\\
{\includegraphics[width=0.25\linewidth]{img_src/mv_comp_pmo/car_28_rgb.png}} &
{\includegraphics[width=0.22\linewidth]{img_src/mv_comp_pmo/car_28_pmo_noise.png}} &
{\includegraphics[width=0.22\linewidth]{img_src/mv_comp_pmo/car_28_pmo.png}} &
{\includegraphics[width=0.22\linewidth]{img_src/mv_comp_pmo/car_28_ours.png}}\\
% {}&{2.483 / 1.343}&{0.484 / 0.468}&{2.522 / 0.474}
\end{tabular}
\vspace{5pt}
\centering
\caption{Comparison on 3D shape prediction from multi-view images on the PMO test set. Our method maintains good surface details, while PMO suffers from the mesh representation and may not effectively optimize the shape.
% The numbers indicates the Chamfer Distance (CD) in direction of pred.$\rightarrow$gt / gt$\rightarrow$pred.. {\color{blue}From the second and fourth row, it can be noticed that CD does not always reflect the quality of the reconstruction.}
}
\label{fig::mv_comp_pmo}
\end{figure}


==> figures/mv_comp_real.tex <==

\begin{figure}[!htb]
\centering
\scriptsize
\setlength\tabcolsep{2.3pt} % default value: 6pt
\begin{tabular}{ccc}
Video sequence & PMO & \textbf{Ours}
\\
{\includegraphics[width=0.35\linewidth]{img_src/mv_comp_real/real_23_rgb.png}} &
{\includegraphics[width=0.28\linewidth]{img_src/mv_comp_real/real_23_pmo.png}} &
{\includegraphics[width=0.28\linewidth]{img_src/mv_comp_real/real_23_ours.png}}
\\
{\includegraphics[width=0.35\linewidth]{img_src/mv_comp_real/real_53_rgb.png}} &
{\includegraphics[width=0.28\linewidth]{img_src/mv_comp_real/real_53_pmo.png}} &
{\includegraphics[width=0.28\linewidth]{img_src/mv_comp_real/real_53_ours.png}}
\\
% {\includegraphics[width=0.35\linewidth]{img_src/mv_comp_real/real_10_rgb.png}} &
% {\includegraphics[width=0.28\linewidth]{img_src/mv_comp_real/real_10_pmo.png}} &
% {\includegraphics[width=0.27\linewidth]{img_src/mv_comp_real/real_10_ours.png}}
\end{tabular}
\vspace{5pt}
\centering
\caption{Comparison on 3D shape prediction from multi-view images on real-world dataset~\cite{choi2016large}. 
It is in general challenging for shape prediction on real image. Comparatively, our method produces more reasonable results with correct structure.
% {\color{blue}Our method may fail either when the provided similarity transform is not accurate or when there are not enough features inside images. Also, it is a really challenging problem under the real-world scenario to initialize the shape code randomly.}
}
\label{fig::mv_comp_real}
\end{figure}


==> figures/supp_depth_completion/table_1201.tex <==
\begin{figure*}[!tb]
\centering
\scriptsize
\setlength\tabcolsep{2.3pt} % default value: 6pt
\begin{tabular}{c|cccccc}
\hline
& dense & 50\% pts & 10\% pts & 100 pts & 50 pts & 20 pts \\
Input depth (direct view) &
{\includegraphics[width=0.12\linewidth]{img_src/supp_depth_completion/table_194/ours_10_direct_points.png}} &
{\includegraphics[width=0.12\linewidth]{img_src/supp_depth_completion/table_194/ours_05_direct_points.png}} &
{\includegraphics[width=0.12\linewidth]{img_src/supp_depth_completion/table_194/ours_01_direct_points.png}} &
{\includegraphics[width=0.12\linewidth]{img_src/supp_depth_completion/table_194/ours_100_direct_points.png}} &
{\includegraphics[width=0.12\linewidth]{img_src/supp_depth_completion/table_194/ours_50_direct_points.png}} &
{\includegraphics[width=0.12\linewidth]{img_src/supp_depth_completion/table_194/ours_20_direct_points.png}}
\\
DeepSDF (direct view) &
{\includegraphics[width=0.12\linewidth]{img_src/supp_depth_completion/table_194/deepsdf_10_direct_output.png}} &
{\includegraphics[width=0.12\linewidth]{img_src/supp_depth_completion/table_194/deepsdf_05_direct_output.png}} &
{\includegraphics[width=0.12\linewidth]{img_src/supp_depth_completion/table_194/deepsdf_01_direct_output.png}} &
{\includegraphics[width=0.12\linewidth]{img_src/supp_depth_completion/table_194/deepsdf_100_direct_output.png}} &
{\includegraphics[width=0.12\linewidth]{img_src/supp_depth_completion/table_194/deepsdf_50_direct_output.png}} &
{\includegraphics[width=0.12\linewidth]{img_src/supp_depth_completion/table_194/deepsdf_20_direct_output.png}}
% \\
% DeepSDF \cite{park2019deepsdf} (second view) &
% {\includegraphics[width=0.12\linewidth]{img_src/supp_depth_completion/table_194/deepsdf_10_az210_output.png}} &
% {\includegraphics[width=0.12\linewidth]{img_src/supp_depth_completion/table_194/deepsdf_05_az210_output.png}} &
% {\includegraphics[width=0.12\linewidth]{img_src/supp_depth_completion/table_194/deepsdf_01_az210_output.png}} &
% {\includegraphics[width=0.12\linewidth]{img_src/supp_depth_completion/table_194/deepsdf_100_az210_output.png}} &
% {\includegraphics[width=0.12\linewidth]{img_src/supp_depth_completion/table_194/deepsdf_50_az210_output.png}} &
% {\includegraphics[width=0.12\linewidth]{img_src/supp_depth_completion/table_194/deepsdf_20_az210_output.png}}
% \\
% DeepSDF \cite{park2019deepsdf} (third view) &
% {\includegraphics[width=0.12\linewidth]{img_src/supp_depth_completion/table_194/deepsdf_10_az120_output.png}} &
% {\includegraphics[width=0.12\linewidth]{img_src/supp_depth_completion/table_194/deepsdf_05_az120_output.png}} &
% {\includegraphics[width=0.12\linewidth]{img_src/supp_depth_completion/table_194/deepsdf_01_az120_output.png}} &
% {\includegraphics[width=0.12\linewidth]{img_src/supp_depth_completion/table_194/deepsdf_100_az120_output.png}} &
% {\includegraphics[width=0.12\linewidth]{img_src/supp_depth_completion/table_194/deepsdf_50_az120_output.png}} &
% {\includegraphics[width=0.12\linewidth]{img_src/supp_depth_completion/table_194/deepsdf_20_az120_output.png}}
\\
Ours (direct view) &
{\includegraphics[width=0.12\linewidth]{img_src/supp_depth_completion/table_194/ours_10_direct_output.png}} &
{\includegraphics[width=0.12\linewidth]{img_src/supp_depth_completion/table_194/ours_womask_05_direct_output.png}} &
{\includegraphics[width=0.12\linewidth]{img_src/supp_depth_completion/table_194/ours_womask_01_direct_output.png}} &
{\includegraphics[width=0.12\linewidth]{img_src/supp_depth_completion/table_194/ours_womask_100_direct_output.png}} &
{\includegraphics[width=0.12\linewidth]{img_src/supp_depth_completion/table_194/ours_womask_50_direct_output.png}} &
{\includegraphics[width=0.12\linewidth]{img_src/supp_depth_completion/table_194/ours_womask_20_direct_output.png}}
% \\
% Ours (second view) &
% {\includegraphics[width=0.12\linewidth]{img_src/supp_depth_completion/table_194/ours_10_az210_output.png}} &
% {\includegraphics[width=0.12\linewidth]{img_src/supp_depth_completion/table_194/ours_womask_05_az210_output.png}} &
% {\includegraphics[width=0.12\linewidth]{img_src/supp_depth_completion/table_194/ours_womask_01_az210_output.png}} &
% {\includegraphics[width=0.12\linewidth]{img_src/supp_depth_completion/table_194/ours_womask_100_az210_output.png}} &
% {\includegraphics[width=0.12\linewidth]{img_src/supp_depth_completion/table_194/ours_womask_50_az210_output.png}} &
% {\includegraphics[width=0.12\linewidth]{img_src/supp_depth_completion/table_194/ours_womask_20_az210_output.png}}
% \\
% Ours (third view) &
% {\includegraphics[width=0.12\linewidth]{img_src/supp_depth_completion/table_194/ours_10_az120_output.png}} &
% {\includegraphics[width=0.12\linewidth]{img_src/supp_depth_completion/table_194/ours_womask_05_az120_output.png}} &
% {\includegraphics[width=0.12\linewidth]{img_src/supp_depth_completion/table_194/ours_womask_01_az120_output.png}} &
% {\includegraphics[width=0.12\linewidth]{img_src/supp_depth_completion/table_194/ours_womask_100_az120_output.png}} &
% {\includegraphics[width=0.12\linewidth]{img_src/supp_depth_completion/table_194/ours_womask_50_az120_output.png}} &
% {\includegraphics[width=0.12\linewidth]{img_src/supp_depth_completion/table_194/ours_womask_20_az120_output.png}}
\\
Ours w. mask (direct view) &
{\includegraphics[width=0.12\linewidth]{img_src/supp_depth_completion/table_194/ours_10_direct_output.png}} &
{\includegraphics[width=0.12\linewidth]{img_src/supp_depth_completion/table_194/ours_05_direct_output.png}} &
{\includegraphics[width=0.12\linewidth]{img_src/supp_depth_completion/table_194/ours_01_direct_output.png}} &
{\includegraphics[width=0.12\linewidth]{img_src/supp_depth_completion/table_194/ours_100_direct_output.png}} &
{\includegraphics[width=0.12\linewidth]{img_src/supp_depth_completion/table_194/ours_50_direct_output.png}} &
{\includegraphics[width=0.12\linewidth]{img_src/supp_depth_completion/table_194/ours_20_direct_output.png}}
% \\
% Ours w. mask (second view) &
% {\includegraphics[width=0.12\linewidth]{img_src/supp_depth_completion/table_194/ours_10_az210_output.png}} &
% {\includegraphics[width=0.12\linewidth]{img_src/supp_depth_completion/table_194/ours_05_az210_output.png}} &
% {\includegraphics[width=0.12\linewidth]{img_src/supp_depth_completion/table_194/ours_01_az210_output.png}} &
% {\includegraphics[width=0.12\linewidth]{img_src/supp_depth_completion/table_194/ours_100_az210_output.png}} &
% {\includegraphics[width=0.12\linewidth]{img_src/supp_depth_completion/table_194/ours_50_az210_output.png}} &
% {\includegraphics[width=0.12\linewidth]{img_src/supp_depth_completion/table_194/ours_20_az210_output.png}}
% \\
% Ours w. mask (third view) &
% {\includegraphics[width=0.12\linewidth]{img_src/supp_depth_completion/table_194/ours_10_az120_output.png}} &
% {\includegraphics[width=0.12\linewidth]{img_src/supp_depth_completion/table_194/ours_05_az120_output.png}} &
% {\includegraphics[width=0.12\linewidth]{img_src/supp_depth_completion/table_194/ours_01_az120_output.png}} &
% {\includegraphics[width=0.12\linewidth]{img_src/supp_depth_completion/table_194/ours_100_az120_output.png}} &
% {\includegraphics[width=0.12\linewidth]{img_src/supp_depth_completion/table_194/ours_50_az120_output.png}} &
% {\includegraphics[width=0.12\linewidth]{img_src/supp_depth_completion/table_194/ours_20_az120_output.png}}
\\
\hline
\end{tabular}
\vspace{5pt}
\centering
\caption{Qualitative comparisons on shape completion under different sparsity of input depth (table).}

\label{fig::supp_depth_completion_table}
\vspace{-5pt}
\end{figure*}

==> figures/supp_mv_pmo.tex <==
% \begin{figure}[!tb]
% \centering
% \scriptsize
% \setlength\tabcolsep{2.3pt} % default value: 6pt
% \begin{tabular}{cccc}
% Video sequence & PMO (rand init)& PMO & \textbf{Ours (rand init)}
% \\
% {\includegraphics[width=0.25\linewidth]{img_src/supp_mv_comp_pmo/chair_1_rgb.png}} &
% {\includegraphics[width=0.24\linewidth]{img_src/supp_mv_comp_pmo/chair_1_pmo_noise.png}} &
% {\includegraphics[width=0.24\linewidth]{img_src/supp_mv_comp_pmo/chair_1_pmo.png}} &
% {\includegraphics[width=0.24\linewidth]{img_src/supp_mv_comp_pmo/chair_1_ours.png}}
% \\
% % {}&{35.744 / 12.213}&{6.656 / 0.505}&{1.425 / 0.397}\\
% {\includegraphics[width=0.25\linewidth]{img_src/supp_mv_comp_pmo/chair_13_rgb.png}} &
% {\includegraphics[width=0.2\linewidth]{img_src/supp_mv_comp_pmo/chair_13_pmo_noise.png}} &
% {\includegraphics[width=0.14\linewidth]{img_src/supp_mv_comp_pmo/chair_13_pmo.png}} &
% {\includegraphics[width=0.16\linewidth]{img_src/supp_mv_comp_pmo/chair_13_ours.png}}
% \\
% % {}&{20.754 / 5.411}&{0.486 / 0.164}&{1.186 / 0.534}\\
% {\includegraphics[width=0.25\linewidth]{img_src/supp_mv_comp_pmo/chair_19_rgb.png}} &
% {\includegraphics[width=0.18\linewidth]{img_src/supp_mv_comp_pmo/chair_19_pmo_noise.png}} &
% {\includegraphics[width=0.2\linewidth]{img_src/supp_mv_comp_pmo/chair_19_pmo.png}} &
% {\includegraphics[width=0.2\linewidth]{img_src/supp_mv_comp_pmo/chair_19_ours.png}}
% \\
% {\includegraphics[width=0.25\linewidth]{img_src/supp_mv_comp_pmo/car_25_rgb.png}} &
% {\includegraphics[width=0.22\linewidth]{img_src/supp_mv_comp_pmo/car_25_pmo_noise.png}} &
% {\includegraphics[width=0.22\linewidth]{img_src/supp_mv_comp_pmo/car_25_pmo.png}} &
% {\includegraphics[width=0.22\linewidth]{img_src/supp_mv_comp_pmo/car_25_ours.png}}
% \\
% {\includegraphics[width=0.25\linewidth]{img_src/supp_mv_comp_pmo/car_34_rgb.png}} &
% {\includegraphics[width=0.22\linewidth]{img_src/supp_mv_comp_pmo/car_34_pmo_noise.png}} &
% {\includegraphics[width=0.22\linewidth]{img_src/supp_mv_comp_pmo/car_34_pmo.png}} &
% {\includegraphics[width=0.22\linewidth]{img_src/supp_mv_comp_pmo/car_34_ours.png}}
% \\
% {\includegraphics[width=0.25\linewidth]{img_src/supp_mv_comp_pmo/car_48_rgb.png}} &
% {\includegraphics[width=0.21\linewidth]{img_src/supp_mv_comp_pmo/car_48_pmo_noise.png}} &
% {\includegraphics[width=0.22\linewidth]{img_src/supp_mv_comp_pmo/car_48_pmo.png}} &
% {\includegraphics[width=0.22\linewidth]{img_src/supp_mv_comp_pmo/car_48_ours.png}}
% \\
% {\includegraphics[width=0.25\linewidth]{img_src/supp_mv_comp_pmo/plane_35_rgb.png}} &
% {\includegraphics[width=0.12\linewidth]{img_src/supp_mv_comp_pmo/plane_35_pmo_noise.png}} &
% {\includegraphics[width=0.2\linewidth]{img_src/supp_mv_comp_pmo/plane_35_pmo.png}} &
% {\includegraphics[width=0.2\linewidth]{img_src/supp_mv_comp_pmo/plane_35_ours.png}}
% \\
% {\includegraphics[width=0.25\linewidth]{img_src/supp_mv_comp_pmo/plane_47_rgb.png}} &
% {\includegraphics[width=0.18\linewidth]{img_src/supp_mv_comp_pmo/plane_47_pmo_noise.png}} &
% {\includegraphics[width=0.2\linewidth]{img_src/supp_mv_comp_pmo/plane_47_pmo.png}} &
% {\includegraphics[width=0.2\linewidth]{img_src/supp_mv_comp_pmo/plane_47_ours.png}}
% \\
% {\includegraphics[width=0.25\linewidth]{img_src/supp_mv_comp_pmo/plane_49_rgb.png}} &
% {\includegraphics[width=0.22\linewidth]{img_src/supp_mv_comp_pmo/plane_49_pmo_noise.png}} &
% {\includegraphics[width=0.24\linewidth]{img_src/supp_mv_comp_pmo/plane_49_pmo.png}} &
% {\includegraphics[width=0.24\linewidth]{img_src/supp_mv_comp_pmo/plane_49_ours.png}}
% \\

% \end{tabular}
% \centering
% \caption{More quatitative comparisons on 3D shape prediction from multi-view images on the PMO test set.}

% \label{fig::supp_mv_comp_pmo}
% \vspace{-5pt}
% \end{figure}

\begin{figure*}[!tb]
\centering
\newcommand{\rgb}{0.22\linewidth}
\scriptsize
\setlength\tabcolsep{6pt} % default value: 6pt
\begin{tabular}{cccc}
Video sequence & PMO (rand init)& PMO & \textbf{Ours (rand init)}
\\
{\includegraphics[width=\rgb]{img_src/supp_mv_comp_pmo/chair_1_rgb.png}} &
{\includegraphics[width=0.24\linewidth]{img_src/supp_mv_comp_pmo/chair_1_pmo_noise.png}} &
{\includegraphics[width=0.22\linewidth]{img_src/supp_mv_comp_pmo/chair_1_pmo.png}} &
{\includegraphics[width=0.22\linewidth]{img_src/supp_mv_comp_pmo/chair_1_ours.png}}
\\
% {}&{35.744 / 12.213}&{6.656 / 0.505}&{1.425 / 0.397}\\
{\includegraphics[width=\rgb]{img_src/supp_mv_comp_pmo/chair_13_rgb.png}} &
{\includegraphics[width=0.18\linewidth]{img_src/supp_mv_comp_pmo/chair_13_pmo_noise.png}} &
{\includegraphics[width=0.12\linewidth]{img_src/supp_mv_comp_pmo/chair_13_pmo.png}} &
{\includegraphics[width=0.14\linewidth]{img_src/supp_mv_comp_pmo/chair_13_ours.png}}
\\
% {}&{20.754 / 5.411}&{0.486 / 0.164}&{1.186 / 0.534}\\
% {\includegraphics[width=0.25\linewidth]{img_src/supp_mv_comp_pmo/chair_19_rgb.png}} &
% {\includegraphics[width=0.18\linewidth]{img_src/supp_mv_comp_pmo/chair_19_pmo_noise.png}} &
% {\includegraphics[width=0.22\linewidth]{img_src/supp_mv_comp_pmo/chair_19_pmo.png}} &
% {\includegraphics[width=0.22\linewidth]{img_src/supp_mv_comp_pmo/chair_19_ours.png}}
% \\
% {\includegraphics[width=0.25\linewidth]{img_src/supp_mv_comp_pmo/car_25_rgb.png}} &
% {\includegraphics[width=0.24\linewidth]{img_src/supp_mv_comp_pmo/car_25_pmo_noise.png}} &
% {\includegraphics[width=0.24\linewidth]{img_src/supp_mv_comp_pmo/car_25_pmo.png}} &
% {\includegraphics[width=0.24\linewidth]{img_src/supp_mv_comp_pmo/car_25_ours.png}}
% \\
{\includegraphics[width=\rgb]{img_src/supp_mv_comp_pmo/car_34_rgb.png}} &
{\includegraphics[width=0.2\linewidth]{img_src/supp_mv_comp_pmo/car_34_pmo_noise.png}} &
{\includegraphics[width=0.2\linewidth]{img_src/supp_mv_comp_pmo/car_34_pmo.png}} &
{\includegraphics[width=0.2\linewidth]{img_src/supp_mv_comp_pmo/car_34_ours.png}}
\\
{\includegraphics[width=\rgb]{img_src/supp_mv_comp_pmo/car_48_rgb.png}} &
{\includegraphics[width=0.18\linewidth]{img_src/supp_mv_comp_pmo/car_48_pmo_noise.png}} &
{\includegraphics[width=0.2\linewidth]{img_src/supp_mv_comp_pmo/car_48_pmo.png}} &
{\includegraphics[width=0.2\linewidth]{img_src/supp_mv_comp_pmo/car_48_ours.png}}
\\
{\includegraphics[width=\rgb]{img_src/supp_mv_comp_pmo/plane_35_rgb.png}} &
{\includegraphics[width=0.11\linewidth]{img_src/supp_mv_comp_pmo/plane_35_pmo_noise.png}} &
{\includegraphics[width=0.18\linewidth]{img_src/supp_mv_comp_pmo/plane_35_pmo.png}} &
{\includegraphics[width=0.18\linewidth]{img_src/supp_mv_comp_pmo/plane_35_ours.png}}
\\
{\includegraphics[width=\rgb]{img_src/supp_mv_comp_pmo/plane_47_rgb.png}} &
{\includegraphics[width=0.16\linewidth]{img_src/supp_mv_comp_pmo/plane_47_pmo_noise.png}} &
{\includegraphics[width=0.18\linewidth]{img_src/supp_mv_comp_pmo/plane_47_pmo.png}} &
{\includegraphics[width=0.18\linewidth]{img_src/supp_mv_comp_pmo/plane_47_ours.png}}
\\
{\includegraphics[width=\rgb]{img_src/supp_mv_comp_pmo/plane_49_rgb.png}} &
{\includegraphics[width=0.2\linewidth]{img_src/supp_mv_comp_pmo/plane_49_pmo_noise.png}} &
{\includegraphics[width=0.22\linewidth]{img_src/supp_mv_comp_pmo/plane_49_pmo.png}} &
{\includegraphics[width=0.21\linewidth]{img_src/supp_mv_comp_pmo/plane_49_ours.png}}
\\
\end{tabular}
\vspace{5pt}
\centering
\caption{More quatitative comparisons on 3D shape prediction from multi-view images on the PMO test set.}

\label{fig::supp_mv_comp_pmo}
% \vspace{-5pt}
\end{figure*}


==> figures/supp_mv_pmo_1201.tex <==

\begin{figure}[!tb]
\centering
\newcommand{\rgb}{0.22\linewidth}
\scriptsize
\setlength\tabcolsep{6pt} % default value: 6pt
\begin{tabular}{cccc}
Video sequence & PMO (rand init)& PMO & \textbf{Ours (rand init)}
\\
{\includegraphics[width=\rgb]{img_src/supp_mv_comp_pmo/chair_1_rgb.png}} &
{\includegraphics[width=0.24\linewidth]{img_src/supp_mv_comp_pmo/chair_1_pmo_noise.png}} &
{\includegraphics[width=0.22\linewidth]{img_src/supp_mv_comp_pmo/chair_1_pmo.png}} &
{\includegraphics[width=0.22\linewidth]{img_src/supp_mv_comp_pmo/chair_1_ours.png}}
\\
% {}&{35.744 / 12.213}&{6.656 / 0.505}&{1.425 / 0.397}\\
% {\includegraphics[width=\rgb]{img_src/supp_mv_comp_pmo/chair_13_rgb.png}} &
% {\includegraphics[width=0.18\linewidth]{img_src/supp_mv_comp_pmo/chair_13_pmo_noise.png}} &
% {\includegraphics[width=0.12\linewidth]{img_src/supp_mv_comp_pmo/chair_13_pmo.png}} &
% {\includegraphics[width=0.14\linewidth]{img_src/supp_mv_comp_pmo/chair_13_ours.png}}
\\
% {}&{20.754 / 5.411}&{0.486 / 0.164}&{1.186 / 0.534}\\
% {\includegraphics[width=0.25\linewidth]{img_src/supp_mv_comp_pmo/chair_19_rgb.png}} &
% {\includegraphics[width=0.18\linewidth]{img_src/supp_mv_comp_pmo/chair_19_pmo_noise.png}} &
% {\includegraphics[width=0.22\linewidth]{img_src/supp_mv_comp_pmo/chair_19_pmo.png}} &
% {\includegraphics[width=0.22\linewidth]{img_src/supp_mv_comp_pmo/chair_19_ours.png}}
% \\
% {\includegraphics[width=0.25\linewidth]{img_src/supp_mv_comp_pmo/car_25_rgb.png}} &
% {\includegraphics[width=0.24\linewidth]{img_src/supp_mv_comp_pmo/car_25_pmo_noise.png}} &
% {\includegraphics[width=0.24\linewidth]{img_src/supp_mv_comp_pmo/car_25_pmo.png}} &
% {\includegraphics[width=0.24\linewidth]{img_src/supp_mv_comp_pmo/car_25_ours.png}}
% \\
{\includegraphics[width=\rgb]{img_src/supp_mv_comp_pmo/car_34_rgb.png}} &
{\includegraphics[width=0.2\linewidth]{img_src/supp_mv_comp_pmo/car_34_pmo_noise.png}} &
{\includegraphics[width=0.2\linewidth]{img_src/supp_mv_comp_pmo/car_34_pmo.png}} &
{\includegraphics[width=0.2\linewidth]{img_src/supp_mv_comp_pmo/car_34_ours.png}}
\\
{\includegraphics[width=\rgb]{img_src/supp_mv_comp_pmo/car_48_rgb.png}} &
{\includegraphics[width=0.18\linewidth]{img_src/supp_mv_comp_pmo/car_48_pmo_noise.png}} &
{\includegraphics[width=0.2\linewidth]{img_src/supp_mv_comp_pmo/car_48_pmo.png}} &
{\includegraphics[width=0.2\linewidth]{img_src/supp_mv_comp_pmo/car_48_ours.png}}
\\
{\includegraphics[width=\rgb]{img_src/supp_mv_comp_pmo/plane_35_rgb.png}} &
{\includegraphics[width=0.11\linewidth]{img_src/supp_mv_comp_pmo/plane_35_pmo_noise.png}} &
{\includegraphics[width=0.18\linewidth]{img_src/supp_mv_comp_pmo/plane_35_pmo.png}} &
{\includegraphics[width=0.18\linewidth]{img_src/supp_mv_comp_pmo/plane_35_ours.png}}
% \\
% {\includegraphics[width=\rgb]{img_src/supp_mv_comp_pmo/plane_47_rgb.png}} &
% {\includegraphics[width=0.16\linewidth]{img_src/supp_mv_comp_pmo/plane_47_pmo_noise.png}} &
% {\includegraphics[width=0.18\linewidth]{img_src/supp_mv_comp_pmo/plane_47_pmo.png}} &
% {\includegraphics[width=0.18\linewidth]{img_src/supp_mv_comp_pmo/plane_47_ours.png}}
\\
{\includegraphics[width=\rgb]{img_src/supp_mv_comp_pmo/plane_49_rgb.png}} &
{\includegraphics[width=0.2\linewidth]{img_src/supp_mv_comp_pmo/plane_49_pmo_noise.png}} &
{\includegraphics[width=0.22\linewidth]{img_src/supp_mv_comp_pmo/plane_49_pmo.png}} &
{\includegraphics[width=0.21\linewidth]{img_src/supp_mv_comp_pmo/plane_49_ours.png}}
\\
\end{tabular}
\vspace{5pt}
\centering
\caption{More quatitative comparisons on 3D shape prediction from multi-view images on the PMO test set.}

\label{fig::supp_mv_comp_pmo}
% \vspace{-5pt}
\end{figure}


==> figures/supp_mv_real.tex <==
\begin{figure*}[!tb]
\centering
\newcommand{\rgb}{0.32\linewidth}
\newcommand{\shape}{0.2\linewidth}
\scriptsize
\setlength\tabcolsep{24pt} % default value: 6pt
\begin{tabular}{ccc}
Video sequence & PMO & \textbf{Ours (rand init)}
\\
{\includegraphics[width=\rgb]{img_src/mv_comp_real/real_21_rgb.png}} &
{\includegraphics[width=\shape]{img_src/mv_comp_real/real_21_pmo.png}} &
{\includegraphics[width=\shape]{img_src/mv_comp_real/real_21_ours.png}}
\\
{\includegraphics[width=\rgb]{img_src/mv_comp_real/real_8_rgb.png}} &
{\includegraphics[width=\shape]{img_src/mv_comp_real/real_8_pmo.png}} &
{\includegraphics[width=\shape]{img_src/mv_comp_real/real_8_ours.png}}
\\
% {\includegraphics[width=\rgb]{img_src/mv_comp_real/real_37_rgb.png}} &
% {\includegraphics[width=\shape]{img_src/mv_comp_real/real_37_pmo.png}} &
% {\includegraphics[width=\shape]{img_src/mv_comp_real/real_37_ours.png}}
% \\
{\includegraphics[width=\rgb]{img_src/mv_comp_real/real_26_rgb.png}} &
{\includegraphics[width=0.15\linewidth]{img_src/mv_comp_real/real_26_pmo.png}} &
{\includegraphics[width=\shape]{img_src/mv_comp_real/real_26_ours.png}}
\\
{\includegraphics[width=\rgb]{img_src/mv_comp_real/real_22_rgb.png}} &
{\includegraphics[width=\shape]{img_src/mv_comp_real/real_22_pmo.png}} &
{\includegraphics[width=\shape]{img_src/mv_comp_real/real_22_ours.png}}
\\
{\includegraphics[width=\rgb]{img_src/mv_comp_real/real_10_rgb_new.png}} &
{\includegraphics[width=0.18\linewidth]{img_src/mv_comp_real/real_10_pmo_new.png}} &
{\includegraphics[width=0.12\linewidth]{img_src/mv_comp_real/real_10_ours_new.png}}
\end{tabular}
\vspace{5pt}
\centering
\caption{More Comparisons on 3D shape prediction from multi-view images on real-world chair dataset~\cite{choi2016large}. 
It is in general challenging for shape prediction on real images. Comparatively, our method produces more reasonable results with correct structure. 
% {\color{blue}Note that similar to PMO, we now also optimize over the similarity transform including rotation, translation and scale, together with the shape code}.
% {\color{red}We show a failure case in the last row. Our method fails when there is insufficient texture on foreground or background as photometric cues. Moreover, our method may fail when the similarity transform is not correctly estimated.}
}
% \vspace{-3pt}
\label{fig::supp_mv_comp_real}
\end{figure*}

% \begin{figure*}[!tb]
% \centering
% \newcommand{\rgb}{0.4\linewidth}
% \newcommand{\shape}{0.25\linewidth}
% \scriptsize
% \setlength\tabcolsep{2.3pt} % default value: 6pt
% \begin{tabular}{ccc}
% Video sequence & PMO & \textbf{Ours (rand init)}
% \\
% {\includegraphics[width=\rgb]{img_src/mv_comp_real/real_21_rgb.png}} &
% {\includegraphics[width=\shape]{img_src/mv_comp_real/real_21_pmo.png}} &
% {\includegraphics[width=\shape]{img_src/mv_comp_real/real_21_ours.png}}
% \\
% {\includegraphics[width=\rgb]{img_src/mv_comp_real/real_8_rgb.png}} &
% {\includegraphics[width=\shape]{img_src/mv_comp_real/real_8_pmo.png}} &
% {\includegraphics[width=\shape]{img_src/mv_comp_real/real_8_ours.png}}
% \\
% {\includegraphics[width=\rgb]{img_src/mv_comp_real/real_37_rgb.png}} &
% {\includegraphics[width=\shape]{img_src/mv_comp_real/real_37_pmo.png}} &
% {\includegraphics[width=\shape]{img_src/mv_comp_real/real_37_ours.png}}
% \\
% {\includegraphics[width=\rgb]{img_src/mv_comp_real/real_26_rgb.png}} &
% {\includegraphics[width=0.18\linewidth]{img_src/mv_comp_real/real_26_pmo.png}} &
% {\includegraphics[width=\shape]{img_src/mv_comp_real/real_26_ours.png}}
% \\
% {\includegraphics[width=\rgb]{img_src/mv_comp_real/real_22_rgb.png}} &
% {\includegraphics[width=\shape]{img_src/mv_comp_real/real_22_pmo.png}} &
% {\includegraphics[width=\shape]{img_src/mv_comp_real/real_22_ours.png}}
% \\
% {\includegraphics[width=\rgb]{img_src/mv_comp_real/real_10_rgb_new.png}} &
% {\includegraphics[width=\shape]{img_src/mv_comp_real/real_10_pmo_new.png}} &
% {\includegraphics[width=0.18\linewidth]{img_src/mv_comp_real/real_10_ours_new.png}}
% \end{tabular}
% \centering
% \caption{More Comparisons on 3D shape prediction from multi-view images on real-world chair dataset~\cite{choi2016large}. 
% It is in general challenging for shape prediction on real image. Comparatively, our method produces more reasonable results with correct structure. 
% % {\color{blue}Note that similar to PMO, we now also optimize over the similarity transform including rotation, translation and scale, together with the shape code}.
% % {\color{red}We show a failure case in the last row. Our method fails when there is insufficient texture on foreground or background as photometric cues. Moreover, our method may fail when the similarity transform is not correctly estimated.}
% }
% % \vspace{-3pt}
% \label{fig::supp_mv_comp_real}
% \end{figure*}



==> tables/table_pix3d_eval.tex <==
\begin{table}[tb]
    \centering
%  	\small
    \begin{tabular}{l|cc}
    \hline
     & EMD & CD$^*$ \\
    \hline
    3D-R2N2~\cite{choy20163d} &  0.211 & 0.239 \\
    PSGN~\cite{fan2017point} & 0.216 & 0.200 \\
    3D-VAE-GAN~\cite{wu2016learning} & 0.176 & 0.182 \\
    DRC~\cite{drcTulsiani17} & 0.144 & 0.160 \\
    MarrNet~\cite{wu2017marrnet} & 0.136 & 0.144 \\
    AtlasNet~\cite{groueix2018atlasnet} & 0.128 & 0.125 \\
    Pix3D~\cite{sun2018pix3d} & 0.124 & 0.124 \\
    ShapeHD~\cite{wu2018learning} & - & 0.123 \\
    ShapeHD \cite{wu2018learning} (infer with gt.) & 0.322 & 0.398 \\
    \hline
    % Ours (mean shape baseline) & 0.134 & 0.170 \\
    % \textbf{Ours} (optimized with pred.) & 0.120 & 0.153 \\
    \textbf{Ours} (optimized with pred.) & 0.141 & 0.153 \\
    % \textbf{Ours} (optimized with gt.) & 0.091 & 0.118 \\
    \textbf{Ours} (optimized with gt.) & \textbf{0.123} & \textbf{0.118} \\
    \hline
    \end{tabular}
    \caption{Quantitative Results of 3D shape reconstruction on Pix3D \cite{sun2018pix3d} dataset. * We follow the same protocol as the baseline implementation \cite{sun2018pix3d} on Chamfer distance implementation, where the L1 distance metric is used.} 
    \label{tab::pix3d_eval}
\end{table}

